Design and implementation of the AMIGA embedded system for data acquisition

The Auger Muon Infill Ground Array (AMIGA) is part of the AugerPrime upgrade of the Pierre Auger Observatory. It consists of particle counters buried 2.3 m underground next to the water-Cherenkov stations that form the 23.5 km$^2$ large infilled array. The reduced distance between detectors in this denser area allows the lowering of the energy threshold for primary cosmic ray reconstruction down to about 10$^{17}$ eV. At the depth of 2.3 m the electromagnetic component of cosmic ray showers is almost entirely absorbed so that the buried scintillators provide an independent and direct measurement of the air showers muon content. This work describes the design and implementation of the AMIGA embedded system, which provides centralized control, data acquisition and environment monitoring to its detectors. The presented system was firstly tested in the engineering array phase ended in 2017, and lately selected as the final design to be installed in all new detectors of the production phase. The system was proven to be robust and reliable and has worked in a stable manner since its first deployment.

==> Makefile <==
# Makefile for building latex documents (c) Darko Veberic
# $Id: Makefile 13341 2020-11-04 11:31:24Z darko $

USEPDFLATEX := 1
USEBIBTEX := 0

TEXFILES := $(shell grep -le '^\s*\\document\(class\|style\)' *.tex)
TARGETS := $(basename $(TEXFILES))
DEPENDENCIES := $(wildcard *.sty *.bib figs/*) $(filter-out $(TEXFILES), $(wildcard *.tex))

##########################################################
SHELL := /bin/bash
PDFS := $(addsuffix .pdf, $(TARGETS))

ifeq (, $(shell which latexmk))
  LATEX := $(if $(filter 1, $(USEPDFLATEX)), pdflatex, latex)
  # 30=black 31=red 32=green 33=yellow 34=blue 35=magenta 36=cyan 37=white 0=cancel
  COLORIZE := awk 'BEGIN{ec="\033[31;1m";wc="\033[34;1m";cc="\033[0m"}/Rerun /||/rerunfilecheck[^.]/{e=e$$0"\n";print ec""$$0""cc;next}/^LaTeX Warning:/||/natbib Warning:/{w=w$$0"\n";print wc""$$0""cc;next}{print}END{if(w||e)print "\n"ec"Warning/error summary:"cc"\n"wc""w""cc;if(e){print ec""e""cc;exit 1}}'
  define basic_latex_rule
    for i in 1 2 3 ; do $(LATEX) $< | $(COLORIZE) && break ; done
  endef
  ifeq ($(USEBIBTEX), 1)
    define latex_rule
      $(LATEX) $< ; bibtex $*
      $(call basic_latex_rule)
    endef
  else
    define latex_rule
      $(call basic_latex_rule)
    endef
  endif
else
  define latex_rule
    latexmk $(if $(filter 1, $(USEPDFLATEX)), -pdf, ) $<
  endef
endif

.PHONY: all clean

all: $(PDFS)

# dependencies
$(PDFS): $(DEPENDENCIES)

clean:
	- $(RM) *{.tex~,.dvi,.log,.aux,.toc,.nav,.out,.snm,.bbl,.blg,.spl,.lof,Notes.bib,.maf,.fff,.lot,.ttt,.bcf,.run.xml,.fdb_latexmk,.fls,.synctex.gz}
	- for f in $(TARGETS) ; do $(RM) $$f{.ps,.pdf} ; done

# general rules
ifeq ($(USEPDFLATEX), 1)
%.pdf: %.tex $(DEPENDENCIES)
	$(call latex_rule)

%.ps: %.pdf
	pdf2ps $<
else
%.dvi: %.tex $(DEPENDENCIES)
	$(call latex_rule)

%.pdf: %.dvi
	dvipdf $<

%.ps: %.dvi
	dvips $< -o
endif

# embed pdf fonts
%.embedded_fonts.pdf: %.pdf
	gs -dSAFER -dNOPLATFONTS -dNOPAUSE -dBATCH -sDEVICE=pdfwrite -sPAPERSIZE=a4 -dCompatibilityLevel=1.4 -dPDFSETTINGS=/printer -dCompatibilityLevel=1.4 -dMaxSubsetPct=100 -dSubsetFonts=true -dEmbedAllFonts=true -sOutputFile=$@ -f $<


==> planIP.tex <==
\begin{table}[H]
\centering
\begin{tabular}{|r|r|r|r|}
\hline
Station & Network          & South                                                                                                     & North                                                                                                     \\ \hline
93      & 10.0.1.0/24 &                                                                                                           & \begin{tabular}[c]{@{}r@{}}m1: 10.0.1.101\\ m2: 10.0.1.102\\ m3: 10.0.1.103\\ m4: 10.0.1.104\end{tabular} \\ \hline
1574    & 10.0.2.0/24 & \begin{tabular}[c]{@{}r@{}}m1: 10.0.1.101\\ m2: 10.0.1.102\\ m3: 10.0.1.103\\ m4: 10.0.1.104\end{tabular} &                                                                                                           \\ \hline
1570    & 10.0.3.0/24 & m1: 10.0.3.101                                                                                            &                                                                                                           \\ \hline
688     & 10.0.4.0/24 & \begin{tabular}[c]{@{}r@{}}m1: 10.0.4.101\\ m2: 10.0.4.102\end{tabular}                                   &                                                                                                           \\ \hline
1764    & 10.0.5.0/24 & \begin{tabular}[c]{@{}r@{}}m1: 10.0.5.101\\ m2: 10.0.5.102\\ m3: 10.0.5.103\\ m4: 10.0.5.104\end{tabular} & \begin{tabular}[c]{@{}r@{}}m1: 10.0.5.105\\ m2: 10.0.5.106\\ m3: 10.0.5.107\\ m4: 10.0.5.108\end{tabular} \\ \hline
1773    & 10.0.6.0/24 & m1: 10.0.6.101                                                                                            &                                                                                                           \\ \hline
1622    & 10.0.7.0/24 & \begin{tabular}[c]{@{}r@{}}m1: 10.0.7.101\\ m2: 10.0.7.102\\ m3: 10.0.7.103\\ m4: 10.0.1.104\end{tabular} & \begin{tabular}[c]{@{}r@{}}m1: 10.0.7.105\\ m2: 10.0.7.106\end{tabular}                                   \\ \hline
\end{tabular}
\caption{IP assignment of each station and its corresponding modules at the Engineering Array at March 2018.}
\label{TAB:ipStation}
\end{table}

==> tablaIP.tex <==
\begin{table}[ht!]
\centering
\label{TAB:ipStation}
\begin{tabular}{|r|r|r|r|r|r|r|}\hline
\multicolumn{1}{|c|}{Station} & \multicolumn{1}{|c|}{\begin{tabular}[c]{@{}c@{}}Distance \\ to axis (m)\end{tabular}} & \multicolumn{1}{|c|}{$\mu$ density $[\frac{\mu}{\SI{}{\metre^2}}]$} & \multicolumn{1}{|c|}{\begin{tabular}[c]{@{}c@{}}M1\\ (10m)\end{tabular}} & \multicolumn{1}{|c|}{\begin{tabular}[c]{@{}c@{}}M2\\ (10m)\end{tabular}} & \multicolumn{1}{|c|}{\begin{tabular}[c]{@{}c@{}}M3\\ (5m)\end{tabular}} & \multicolumn{1}{|c|}{\begin{tabular}[c]{@{}c@{}}M4 \\ (5m)\end{tabular}} \\\hline
1570 south    & 471.1        & -            & -               & -           \\\hline
1622 south    & 33.7         & 29.4         & 10.1            & 11.3        \\\hline
1622 north    & 34.7         & 25.0         & -               & -           \\\hline
688 south     & 41.8         & 24.8         & -               & -           \\\hline
1574 south    & 19.7         & 25.0         & 9.2             & 12.2        \\\hline
1764 south    & 4.0          & 5.0          & 3.0             & 1.0         \\\hline
1764 north    & 6.1          & 3.0          & 1.0             & 4.0         \\\hline
93 north      & 1.0          & 2.0          & 1.0             & 3.0         \\\hline
1773 south    & 0.0          & -            & -               & -           \\\hline
\end{tabular}
\caption{Key event data calculated for the presented event, separated by station, and analysing twin detectors separately.}
\end{table}

==> table_power.tex <==
\begin{table}[ht]
\centering
\begin{tabular}{|r|r|r|}
\hline
\multicolumn{1}{|l|}{\textbf{Voltage [V]}} & \multicolumn{1}{l|}{\textbf{Current [mA]}} & \multicolumn{1}{l|}{\textbf{Power [W]}} \\ \hline
24      & 75    & 1.800   \\ \hline
3.3     & 210   & 0.693   \\ \hline
1.8     & 44    & 0.079   \\ \hline
2.5     & 46    & 0.115   \\ \hline
1.2     & 236   & 0.283   \\ \hline
\end{tabular}
\caption{Power consumption for each of the outputs shown in figure \ref{{FIG:PWRSUP}}.}
\label{TAB:LUTCount}
\end{table}


